An Empirical Review of Model-based Adaptive Sampling for Global Optimization of Expensive Black-box Functions

This paper reviews the state-of-the-art model-based adaptive sampling approaches for single-objective black-box optimization (BBO). While BBO literature includes various promising sampling techniques, there is still a lack of comprehensive investigations of the existing research across the vast scope of BBO problems. We first classify BBO problems into two categories: engineering design and algorithm design optimization and discuss their challenges. We then critically discuss and analyze the adaptive model-based sampling techniques focusing on key acquisition functions. We elaborate on the shortcomings of the variance-based sampling techniques for engineering design problems. Moreover, we provide in-depth insights on the impact of the discretization schemes on the performance of acquisition functions. We emphasize the importance of dynamic discretization for distance-based exploration and introduce EEPA+, an improved variant of a previously proposed Pareto-based sampling technique. Our empirical analyses reveal the effectiveness of variance-based techniques for algorithm design and distance-based methods for engineering design optimization problems.

==> SO.tex <==
\section{Surrogate Optimization}

% \begin{algorithm}[!tb]
% \caption{{\bf Generic Surrogate Optimization}}
% \begin{algorithmic}[1]
% \label{alg:SurOpt}

% \STATE $\mathcal{D}=\{\mathbf{x}^1, \ldots, \mathbf{x}^{n_0}\}$, a set of $n_0$ labeled points, selected by a DOE method \label{step1}

% \STATE $\mathcal{F}= \{f(\mathbf{x}^i)|\mathbf{x}^i\in \mathcal{D}\}$ \label{step2}
% \WHILE {Termination criteria not satisfied}
%  \STATE \emph{Surrogate}: Fit a surrogate model $\hat{f}$ on $(\mathcal{D},\mathcal{F})$\label{step4} 
%  \STATE \emph{Sampling}: Determine new candidate points, $S$\label{step5}
%  \STATE \emph{Evaluation}: $\mathcal{F}_S=\{f(\mathbf{x}^i)|\mathbf{x}^i\in S\}$ 
%  \label{step6}
%   \STATE $\mathcal{D}= \mathcal{D}\cup \mathcal{S}$; $\mathcal{F}=\mathcal{F}\cup \mathcal{F}_S$
%  \STATE $\mathbf{x}^o\in\argmin_{\mathbf{x}\in \mathcal{D}} f(\mathbf{x})$\label{step8}
% \ENDWHILE
% \STATE Return $\mathbf{x}^*=\mathbf{x}^o$
% \end{algorithmic}
% \end{algorithm}

\subsection{EEPA}

\subsection{Dycors}

\subsection{SOP}


